Computations of quantum Giambelli formulas in some exceptional homogeneous spaces

This paper gathers results obtained with a software written in Java. For exceptional minuscule, quasi-minuscule, cominuscule or adjoint homogeneous spaces, the Schubert cells are expressed as polynomials in the generators of the quantum cohomology algebra.

==> tableau-e6p2-8-2-1.tex <==
%% GENERATED BY QUIVER CALCULUS


\begin{pspicture*}(0,0)(3.0,2.4)

\psline(0.699,0.099)(1.101,0.501)
\psline(0.501,0.099)(0.099,0.501)
\psellipse(0.6,0.0)(0.14,0.14)
\put(0.54,0.0){4}
\psline(1.101,0.699)(0.699,1.101)
\psline(1.299,0.699)(1.701,1.101)
\psellipse(1.2,0.6)(0.14,0.14)
\put(1.14,0.6){2}
\psline(2.301,0.699)(1.899,1.101)
\psellipse(2.4,0.6)(0.14,0.14)
\put(2.34,0.6){3}
\psline(0.099,0.699)(0.501,1.101)
\psellipse(0.0,0.6)(0.14,0.14)
\put(-0.06,0.6){1}
\psline(0.699,1.299)(1.101,1.701)
\psellipse[fillstyle=solid,fillcolor=black](0.6,1.2)(0.14,0.14)
\psline(1.701,1.299)(1.299,1.701)
\psellipse[fillstyle=solid,fillcolor=black](1.8,1.2)(0.14,0.14)
\psline(1.2,1.94)(1.2,2.26)
\psellipse[fillstyle=solid,fillcolor=black](1.2,1.8)(0.14,0.14)
\psellipse[fillstyle=solid,fillcolor=black](1.2,2.4)(0.14,0.14)

